Understanding team collapse via probabilistic graphical models

In this work, we develop a graphical model to capture team dynamics. We analyze the model and show how to learn its parameters from data. Using our model we study the phenomenon of team collapse from a computational perspective. We use simulations and real-world experiments to find the main causes of team collapse. We also provide the principles of building resilient teams, i.e., teams that avoid collapsing. Finally, we use our model to analyze the structure of NBA teams and dive deeper into games of interest.

==> sections/learning_experiments.tex <==
\section{Learning from synthetic data}
In this section we test the EM learning algorithm, described in section \ref{sec: learning}, on synthetic data.

We create a model with $5$ entities and the following parameters:
\begin{align}
    \vect{M} = 
    \begin{bmatrix}
        0.8 & 0.2 & 0 \\
        0.2 & 0.8 & 0.2 \\
        0 & 0.2 & 0.8
    \end{bmatrix},
\end{align}
\begin{align}
    \vect{N} = 
    \begin{bmatrix}
        0.7 & 0.2 & 0.1 \\
        0.2 & 0.6 & 0.2 \\
        0.1 & 0.2 & 0.7
    \end{bmatrix},
\end{align}
\begin{align}
    \vect{E} = 
    \begin{bmatrix}
        0.8 & 0.2 & 0 \\
        0.2 & 0.8 & 0.2 \\
        0 & 0.2 & 0.8
    \end{bmatrix},
\end{align}
and
\begin{align}
    \vect{R}^1 &= (1, 0, 0, 0, 0, 0) \\
    \vect{R}^i &= (0, 1, 0, 0, 0, 0), \forall i \in \{2, 3, 4, 5\}.
\end{align}.

We generate $100$ samples and run the EM algorithm. Our primary goal is to identify the team structure as captured by $\vect{R}$ (see Experiments section). As a secondary goal we want to learn the rest of the parameters. We randomly initialize $\vect{M}$, $\vect{N}$, $\vect{E}$ and $\vect{R}^i = (1/6, 1/6, 1/6, 1/6, 1/6, 1/6), \forall i \in [5]$.
Our learned parameters are the following:
\begin{align}
    \vect{M} = 
    \begin{bmatrix}
        1 & 0 & 0 \\
        0 & 1 & 0 \\
        0 & 0 & 1
    \end{bmatrix},
\end{align}
\begin{align}
    \vect{N} = 
    \begin{bmatrix}
        0.22 & 0.78 & 0 \\
        0.04 & 0.87 & 0.09 \\
        0 & 0.49 & 0.5
    \end{bmatrix},
\end{align}
\begin{align}
    \vect{E} = 
    \begin{bmatrix}
        0.59 & 0.41 & 0 \\
        0.12 & 0.75 & 0.13 \\
        0.01 & 0.23 & 0.75
    \end{bmatrix},
\end{align}
\begin{align}
    \vect{R}^1 &= (0.16, 0.5, 0.1, 0.24, 0,  0.01)\\
    \vect{R}^2 &= (0.09, 0.66, 0.03, 0.2,  0.02, 0) \\
    \vect{R}^3 &= (0.14, 0.67, 0.13, 0.04, 0.01, 0) \\
    \vect{R}^4 &= (0.13, 0.75, 0.01, 0.05, 0.07, 0) \\
    \vect{R}^5 &= (0.33, 0.38, 0.06, 0.1,  0.13, 0.01).
\end{align}
Observe that the model has correctly learned that player $1$ is heavily dependent on him/her self, while other players are mostly dependent on player $1$.
The negative log-likelihood of the model defined from the aforementioned parameters is $414$, while the negative log-likelihood of the true model is $417$ (larger than that of the learned model).

We emphasize the crucial role of initialization. Specifically, we found out that EM may converge to radically different parameters depending on the initialization. Moreover, we note that many different sets of parameters may explain the data and achieve low negative-log-likelihood.
Due to the above complications, in section \ref{sec: real-world experiments}, we develop a more practical approach. Namely, we generate a database of possible parameter configurations. Given a set of observations we calculate the negative log-likelihood of each parameter configuration and select the one that achieves the minimum.


==> sections/related.tex <==
\section{Related work}

%Sports have traditionally served as a testbed for examining various behavioral economics hypotheses such as the winner's curse, risk aversion and decision making, implicit biases in judgment, and others \cite{massey2013loser,romer2006firms,pelechrinis2023quantifying}. 
%Sports is also a natural environment to study performance and decision making under pressure.
%However, 
During the last decade, the ability to collect player tracking spatio-temporal data has led to a growth on computational approaches for evaluating players and team strategy in a variety of sports. 
Several applications have been developed and introduced ranging from spatial metrics for evaluating the defensive performance of players/teams \cite{miller14,nguyen2023here,lucey2014quality}, to computational models for estimating the expected points/goals added by different actions happening on the court/pitch \cite{yue2014learning,damour15,cervone2016multiresolution,decroos2019actions,yurko2020going,sicilia2019deephoops}, to generative models for generating player trajectories to simulate team actions \cite{chen2021instant,seidl2018bhostgusters}. 
Our work falls into this general area. Below, we summarize how our work relates to existing work on different aspects of sport analytics. 
We also connect our work to existing work on probabilistic models and interconnected Hidden Markov Models (HMMs) in particular.

\iffalse
For example, Bransen {\em et al.} \cite{bransen2019choke} develop appropriate metrics to evaluate the performance of individual soccer players under situations with high mental pressure. 
The latter includes pre-game pressure (e.g., a game of high importance) and in-game pressure (e.g., a crucial moment in the game). 
Dohmen \cite{dohmen2008professionals} focused on studying penalty shootouts and he found that players of the home team are more likely to choke, while at the same time the study identified no evidence in their data that high stakes induce choking. 
A detailed overview on the mechanisms and potential moderators of choking in sport, along with possible  interventions alleviate it is further provided by Hill {\em et al.} \cite{hill2010choking}. 
In this work, we enhance this literature by studying the {\em team effects} of individual performance, as well as, the possible influence they exert on the performance of their teammates and how this translates to a team's ability to withstand, or not, periods of subpar performance of individual players. 
\fi

\spara{Sports analytics, team and player performance:} One of the main tasks that the field of sports analytics has dealt with is that of team and player performance evaluation. 
This typically is achieved through models that learn team and player ratings. 
These ratings have several applications ranging from match prediction and gambling to helping teams identify players to acquire who are undervalued using traditional statistics. 
The simplest team ratings are based on regression methods, where the score differential is modeled as a function of the home and visiting team \cite{langville2012s,w2007quantile,bradley1952rank,winston2022mathletics}. 
Network-based ratings and rankings have also been developed, analyzing a ``who-wins-whom'' network, and provides a better ranking for teams as compared to rankings based on win-loss record \cite{park2005network,pelechrinis2016sportsnetrank}, while latent space models have also been used to learn an embedding for each team that will help obtain a team ranking \cite{chen2016modeling,chen2016predicting,pelechrinis2018linnet}. 
Similarly, for evaluating players the traditional approach for obtaining player ratings is using regression based approaches \cite{macdonald2011regression,thomas2013competing,sabin2021estimating} to model the score differential during a game possession as a function of the players on the court/pitch. 

These ratings do not incorporate any dependencies between the players and make the implicit assumptions that player ratings are additive, {\ie}, a team is the sum of the individual players. 
As such, it is hard for these type of models to help us understand and explain situations where a team significantly over or under performs its expectation within a game. 
In our work, we explicitly consider the  dependencies between players and we develop a framework that can explain how these dependencies can lead to a team collapsing. 

\spara{Performing under pressure and ``choking''}: The common belief is that super-star athletes shine when the stakes are high, while athletes in lower tiers severely under perform under pressure, {\ie}, they ``choke'' or collapse. 
While there has been some literature on players performance and decision-making under pressure, this has traditionally been in the field of sports psychology \cite{baumeister1986review,pineda2022play,parkin2017gunslingers}. 
The vast majority of the literature has been on the {\em complementary} phenomenon of ``clutch'' players, {\ie}, players that deliver when the stakes are high. 
The majority of this literature indicates that individual clutch performance is highly noisy \cite{solomonov2015clutch,wallace2013homo,birnbaum2008clutch}. 
One of the few computational studies on player performance under pressure is that from Bransen {\etal}~\cite{bransen2019choke} who develop appropriate metrics to evaluate the performance of individual soccer players under situations with high mental pressure. 
%The latter includes pre-game pressure (e.g., a game of high importance) and in-game pressure (e.g., a crucial moment in the game). 
In a similar direction, Dohmen \cite{dohmen2008professionals} focused on studying penalty shootouts and found that players of the home team are more likely to choke, while at the same time the study identified no evidence in their data that high stakes induce choking. 
A detailed overview on the mechanisms and potential moderators of choking in sport, along with possible  interventions to alleviate it is further provided by Hill {\etal}~\cite{hill2010choking}. 

In our work, we enhance this literature by studying the {\em team effects} of individual performance, as well as, the possible influence they exert on the performance of their teammates and how this translates to a team's ability to withstand, or not, periods of subpar performance of individual players. 


\spara{Computational work on interacting HMMs}
\note[ET]{Iasona can you please add some related work on this}

==> sections/team-collapse.tex <==
%\section{Team collapse}


